Numerical simulation of hot accretion flows (IV): effects of black hole spin and magnetic field strength on the wind and the comparison between wind and jet properties

This is the fourth paper of our series of works studying winds from hot accretion flows around black holes. In the first two papers, we have shown the existence of strong winds in hot accretion flows using hydrodynamical and magnetohydrodynamical (MHD) simulations. In the third paper, by using three dimensional general relativity MHD numerical simulation data of hot accretion flows and adopting a "virtual particle trajectory" data analysis approach, we have calculated the properties of wind, such as its mass flux and velocity. However, that paper focuses only on a non-spinning black hole and SANE (standard and normal accretion). In the present paper, we extend the third paper by including cases of a rapidly rotating black hole and MAD (magnetically arrested disk). We focus on investigating the effect of spin and magnetic field on the properties of wind and jet. It is found that a larger spin and stronger magnetic field usually enhance the wind and jet. The formulae describing the mass flux, poloidal velocity, and fluxes of momentum, kinetic energy, and total energy of wind and jet are presented. One interesting finding, among others, is that even in the case of very rapidly spinning black hole where the jet is supposed to be the strongest, the momentum flux of jet is smaller than that of wind, while the total energy flux of jet is larger than that of wind by at most a factor of 10. This result suggests that wind potentially plays a more important role than jet at least for some problems in active galactic nuclei feedback.

==> figure/psbbox <==
#! /bin/sh

# psbbox
# calculates the BoundingBox for a PostScript file
# optionally prints it, fixes it in the file, or puts it in a .bb file

# CURRENTLY WORKS ON SINGLE-PAGE FILES ONLY!
# TO DO: use mpage to separate out all the pages in each file,
# calculate the boxes, and reassemble with mpage again

# Joe Harrington <jh@alum.mit.edu> Sat Mar 17 13:22:36 EST 2001
# version 0.2
# Usage:
# psbbox [-fix] [-file] [-noprint] <file>...

fix=0
file=0
print=1
exitstat=0

while [ "$*" != "" ]; do
  if [ "$1" = "-fix" ]; then
    fix=1
  elif [ "$1" = "-file" ]; then
    file=1
  elif [ "$1" = "-noprint" ]; then
    print=0
  elif [ "$1" = "--help" ]; then
    echo 'psbbox [-fix] [-file] [-noprint] <file>...'
  elif [ "$1" = "--version" ]; then
    echo 'psbbox version 0.02 2001-Mar-17'
  else
    psfiles=$psfiles" "$1
  fi
  shift
done

for i in $psfiles; do
  base=`basename $i .gz`
  reader=cat
  writer=cat
  if [ $base != $i ]; then
    reader=zcat
    writer=gzip
  fi

  $reader $i \
    | gs -q -dNOPAUSE -dBATCH -sDEVICE=bbox -f - \
    > ${base}.bb$$ 2>&1

  grep %%BoundingBox: ${base}.bb$$ > /dev/null
  if [ $? = 1 ]; then
    echo "psbbox: $i: BoundingBox not computed by Ghostscript." 1>&2
    echo "        Make sure there is a \"showpage\"." 1>&2
    exitstat=1
  fi

  # print what we got
  if [ $print = 1 ]; then
    cat ${base}.bb$$
  fi

  # fix the bounding box in the file if wanted
  if [ $fix = 1 ]; then
    # correct info
    bbox=`grep %%BoundingBox: ${base}.bb$$ | head -1`
    hbox=`grep %%HiResBoundingBox: ${base}.bb$$ | head -1`
    # ghostscript doesn't produce a PageBoundingBox
    pbox=`echo $bbox | sed s/%%BoundingBox/%%PageBoundingBox/`

    # locations in the file (read only once in case it's big)
    $reader $i | egrep -n '%%.*BoundingBox:' > ${base}.obb$$
    bbno=`grep      %%BoundingBox: ${base}.obb$$ | head -1 | sed 's/:.*//'`
    hbno=`grep %%HiResBoundingBox: ${base}.obb$$ | head -1 | sed 's/:.*//'`
    pbno=`grep  %%PageBoundingBox: ${base}.obb$$ | head -1 | sed 's/:.*//'`

    # sed commands and default locations for new lines
    bcmd=c
    hcmd=c
    pcmd=c
    if [ "$bbno" = "" ]; then
      bbno=2
      bcmd=i
    fi
    if [ "$hbno" = "" ]; then
      hbno=`expr $bbno + 1`
      hcmd=i
    fi

    # Don't add a PageBoundingBox unless there already is one.  If you
    # can figure out how to do this in a single sed command line that
    # doesn't add at least a blank line (rather than the repetition in
    # the conditional below), please tell me.
    if [ "$pbno" = "" ]; then
      $reader $i \
        | sed -e "$bbno $bcmd \\
$bbox" \
	      -e "$hbno $hcmd \\
$hbox" \
      | $writer \
      > $i.tmp
    else
      $reader $i \
        | sed -e "$bbno $bcmd \\
$bbox" \
	      -e "$hbno $hcmd \\
$hbox" \
	      -e "$pbno $pcmd \\
$pbox" \
      | $writer \
      > $i.tmp
    fi
    if [ $? = 0 ]; then
      mv $i.tmp $i
    fi
  fi

  # create a .bb file if wanted
  if [ $file = 1 ]; then
    cp -p ${base}.bb$$ ${base}.bb
  fi

  # clean up
  rm -f ${base}.bb$$ ${base}.obb$$
done

exit $exitstat

